LitGen: Genetic Literature Recommendation Guided by Human Explanations

As genetic sequencing costs decrease, the lack of clinical interpretation of variants has become the bottleneck in using genetics data. A major rate limiting step in clinical interpretation is the manual curation of evidence in the genetic literature by highly trained biocurators. What makes curation particularly time-consuming is that the curator needs to identify papers that study variant pathogenicity using different types of approaches and evidences---e.g. biochemical assays or case control analysis. In collaboration with the Clinical Genomic Resource (ClinGen)---the flagship NIH program for clinical curation---we propose the first machine learning system, LitGen, that can retrieve papers for a particular variant and filter them by specific evidence types used by curators to assess for pathogenicity. LitGen uses semi-supervised deep learning to predict the type of evidence provided by each paper. It is trained on papers annotated by ClinGen curators and systematically evaluated on new test data collected by ClinGen. LitGen further leverages rich human explanations and unlabeled data to gain 7.9%-12.6% relative performance improvement over models learned only on the annotated papers. It is a useful framework to improve clinical variant curation.

==> method.tex <==
\section{Method}

\james{This Methods section is quite confusing and needs to be rewritten. It's not clear from the text how the explanation and unlabeled data are used. Reduce the space and clutter that's spend on the standard concepts (e.g. LSTM, gradient descent) and use it to more precisely define the new ideas. Please refer back to the outline we wrote on my whiteboard. }


We propose two methods to incorporate high-level explanations into both supervised learning and proxy-label semi-supervised learning. We show that adding explanations to both settingsss can effectively improve the performance of the final model and we describe them in details in the following sections.

% We propose two learning paradigms to leverage the extra information provided by explanations: supervised learning and proxy-label approaches for semi-supervised learning. 

We use the following notations to describe our data. Each paper is associated with an explanation on why it is chosen as a relevant literature for a VCI tab. Explanations are entered by curators manually. For the labeled papers dataset, we have $(x, \bm{y}) \in (\mathcal{X}, \bm{\mathcal{Y}})$ where $\bm{y} \in [0, 1]^m$ for m labels and $|\bm{y}| = m$. This is a multi-label setting to capture the fact that each paper can be submitted to multiple VCI tabs. The human explanation dataset can be described as $(e, y) \in (E, \mathcal{Y})$, where $y \in \{1,...,m\}$ and $|y| = 1$ because each explanation can only be associated with one VCI tab. Since both explanations and papers are submitted to the same set of tabs, $\mathcal{Y}$ and $\bm{\mathcal{Y}}$ share label space.

\subsection{Learning from labeled data}

\paragraph{LitGen model}

We use the state-of-the-art text processing algorithm for our recommendation model: Long-short-term memory networks (LSTM). It has been widely used in many natural language processing applications~\cite{hochreiter1997long,mikolov2012statistical} and recently adopted for clinical long text processing~\cite{nie2018deeptag,zhang2019vettag}. 

A long-short-term memory network is a recurrent neural network with a long-short-term memory cell. It takes one word as input, as well as the previous cell and hidden state. Given a sequence of word embeddings $x_1, ..., x_T$,  an LSTM network computes these inputs recurrently and outputs a sequence of vectors $h_1, ..., h_T$.
An extension of the LSTM network is to intorduce bidirectional passes~\cite{graves2005bidirectional}. We adopt this extension. At the end of both passes, bidirectional LSTM will output two hidden states represents each input $x_t$, and we stack these two hidden states as our new hidden state for this input $ h_t = [\overrightarrow{h_t};\overleftarrow{h_t}]$.

%the recurrent computation of LSTM network at a time step $t$ can be described in Eq 1-7, where $\sigma$ is the sigmoid function $\sigma = 1 / (1 + e^{-x})$, and $\tanh$ is the hyperbolic tangent function. We use $\odot$ to indicate the hadamard product.

% \begin{equation}
% \begin{split}
% f_t & = \sigma(W_f x_t + V_f h_{t - 1} + b_f) \\
% i_t & = \sigma(W_i x_t + V_i h_{t - 1} + b_i) \\
% o_t & = \sigma(W_o x_t + V_o h_{t - 1} + b_o) \\
% \tilde{c}_t & = \tanh(W_c x_t + V_c h_{t - 1} + b_c) \\
% c_t & = f_t \odot c_{t - 1} + i_t \odot \tilde{c}_t \\
% h_t & = o_t \odot \tanh(c_t)
% \end{split}
% \label{eq:lstm}
% \end{equation}

%\begin{eqnarray}
%f_t & = \sigma(W_f x_t + V_f h_{t - 1} + b_f) \\
%i_t & = \sigma(W_i x_t + V_i h_{t - 1} + b_i) \\
%o_t & = \sigma(W_o x_t + V_o h_{t - 1} + b_o) \\
%\tilde{c}_t & = \tanh(W_c x_t + V_c h_{t - 1} + b_c) \\
%c_t &= f_t \odot c_{t - 1} + i_t \odot \tilde{c}_t \\
%h_t &= o_t \odot \tanh(c_t) \\
%\end{eqnarray}

%An extension of this recurrent neural network with LSTM cell is to introduce bidirectional passes \cite{graves2005bidirectional}. Graves et al. shows that introducing bidrectional passes, it can effectively eliminate problems such as retaining long-term dependency when the document is very long. We parameterize two LSTM cells with different set of parameters, one cell is used in forward pass where the sequence is passed in sequentially from the beginning $\{x_1, ..., x_T\}$ , one cell is used for backward pass, where the sequence is passed in with reversed ordering $\{x_T, ..., x_1\}$. At the end of both passes, bidirectional LSTM will output two hidden states represents each input $x_t$, and we stack these two hidden states as our new hidden state for this input $ h_t = [\overrightarrow{h_t};\overleftarrow{h_t}]$.

After computing hidden states over the entire document, we introduce global max pooling over the hidden states, as suggested by Collobert \& Weston \cite{collobert2008unified} so that the hidden states will aggregate information from the entire documents. Assuming the dimension of hidden state is $d$, global max pooling apply an element-wise maximum operation over the temporal dimension of the hidden state matrix, described in Eq~1-2.

% \begin{equation}
% \begin{aligned}
% H &= [h_1, ..., h_T] \text{, } H \in \reals^{T \times d} \\
% c_j &= \max(H_{j}) \text{, for } j = 1, ..., d\\
% \end{aligned}
% \label{eq:gmp}
% \end{equation}

% ha...I'm really not sure which part is really undefined...all worked
\begin{eqnarray}
H &= [h_1, ..., h_T] \text{, } H \in \reals^{T \times d} \\
c_j &= \max(H_{j}) \text{, for } j = 1, ..., d
\end{eqnarray}

Then we define a binary classifier for each of VCI tab. This serves as our baseline model. The binary classifier takes in a vector $\bm{c}$ that represents the veterinary record and outputs a sufficient statistic for the Bernoulli probability distribution indicating the probability of whether a paper belongs to a VCI tab. For $i = 1, ..., m$ with input $x$:

\begin{equation}
\begin{aligned}
P(y_i) = \hat{y}_i = \sigma(\theta_i^\intercal \bm{c}(x))\\
\end{aligned}
\label{eq:binary}
\end{equation}

\subsection{Learning from labeled data with explanations}

% So use: MTL Exp + ClinGen + Unsup (directly fine-tune this model on unsup, simplest way to combine all three)
% how to use explanations on unlabeled data

\begin{figure}[h]
\centerline{
\includegraphics[scale=0.4]{images/WeakSupFigure4.pdf} % [width=4.5cm]
}
\caption{Multi-task learning pipeline that leverages labeled data and explanations}
\label{fig:mtl-pipeline}
\end{figure}

A simple algorithm that allows model to learn both from the labeled papers and human explanations is multi-task learning. We use the LitGen model as described above. We can formulate two tasks on two datasets: one is to recommend paper to the correct set of VCI tabs, another is to find out which tab does the explanation belong. For the paper recommendation task, we use parameter $\Theta$ for the classifier, and for the explanation classification task, we use parameter $\Gamma$ for the classifier. Both tasks share the same LSTM model for text processing.

\begin{eqnarray}
 \log P(\bm{y}|x) &= \log \sum_{i=1}^m \sigma(\theta_i^\intercal \bm{c}(x)), \theta_i \in \Theta \\
\mathcal{L}_1 &= \sum_{x, \bm{y} \in \mathcal{X}, \bm{\mathcal{Y}}} \log P(\bm{y}|x) \\
 \log P(y|e) &= \log \sum_{i=1}^m \sigma(\gamma_i^\intercal \bm{c}(e)), \gamma_i \in \Gamma \\
\mathcal{L}_2 &= \sum_{e, y \in E, \mathcal{Y}} \log P(y|e) \\
\mathcal{L} &= \mathcal{L}_1 + \lambda * \mathcal{L}_2
\end{eqnarray}

For each epoch, we first train on one task with minibatch optimization, and when it has finished, we train on the task. Since $\mathcal{L}_2$ is not associated with the real task, we add a scalar $\lambda \in [0, 1]$ to scale down the loss. We describe the training procedure with the following pseudo-code:

% \newcommand{\keyw}[1]{{\bf #1}}
% {
% \small{
% \begin{tabbing}
% \quad \=\quad \=\quad \kill
% \keyw{while} epoch $<$ K \\
% \> \keyw{for} x, $\bm{y}$ \keyw{in} $\mathcal{X}, \bm{\mathcal{Y}}$ do \\
% \> \> $\bm{c}(x)$ = LitGen(x) \\
% \> \> $\mathcal{L}_1$ =  $\log P(\bm{y}|x)$ \\
% \> \> Run a gradient descent step on $\mathcal{L}_1$ \\
% \> \keyw{for} e, y \keyw{in} $E, \mathcal{Y}$ do \\
% \> \> $\bm{c}(e)$ = LitGen(e) \\
% \> \> $\mathcal{L}_2$ =  $\log P(y|e)$ \\
% \> \> Run a gradient descent step on $\lambda * \mathcal{L}_2$ \\
% \> epoch = epoch + 1 \\
% \keyw{return} LitGen
% \end{tabbing}
% }
% }

\begin{algorithm}[H]
\caption{Training Procedure for Multi-task Learning}
\begin{algorithmic}
\While {epoch $<$ K} 
\ForAll{x, $\bm{y}$ $\in$ $\mathcal{X}, \bm{\mathcal{Y}}$} 
\State $\bm{c}(x) \gets$ LitGen(x) 
\State $\mathcal{L}_1 \gets \log P(\bm{y}|x)$
\State take gradient step on $\mathcal{L}_1$
\EndFor
\ForAll{e, y $\in$ $E, \mathcal{Y}$} 
\State $\bm{c}(e) \gets$ LitGen(e) 
\State $\mathcal{L}_2 \gets \log P(y|e)$
\State take gradient step on $\lambda * \mathcal{L}_2$
\EndFor
epoch $\gets$ epoch + 1
\EndWhile
\end{algorithmic}
\end{algorithm}

This simple approach has a few drawbacks. The length of explanations is considerably shorter than paper abstract. The model is trained under two sets of data with distributional shift on the input. The output distribution between two datasets are also different. Explanations' labels are mutually exclusive (i.e., one explanation can only be used for one VCI tab), while papers' labels are non-mutually exclusive (i.e., one paper can be submitted to multiple VCI tabs).

% We process the paper and obtain the vector representation $\bm{c}$ and predict whether a paper is recommended in a VCI tab. In addition, we process the short explanations and obtain its representation $\bm{e}$ similar to how we processed papers and use a separate classifier to predict whether an explanation text is obtained from a VCI tab.

% \newcommand{\keyw}[1]{{\bf #1}}
% {
% \small{
% \begin{tabbing}
% \quad \=\quad \=\quad \kill
% \keyw{while} epoch $<$ K \\
% \> \keyw{for} x, $\bm{y}$ \keyw{in} $\mathcal{X}, \bm{\mathcal{Y}}$ do \\
% \> \> $\bm{c}$ = LitGen(x) \\
% \> \> $\mathcal{L}_1$ = BCE($\hat{\bm{y}}$, $\bm{y}$) \\
% \keyw{return} $E$
% \end{tabbing}
% }
% }

% \newcommand{\keyw}[1]{{\bf #1}}
% \begin{tabbing}
% \quad \=\quad \=\quad \kill
% \keyw{for} each $x$ \keyw{do} \\
% \> \keyw{if} extension$(p, x)$ \\
% \> \> \keyw{then} $E:=E\cup\{x\}$\\
% \keyw{return} $E$
% \end{tabbing}


% \begin{algorithm}[H]
%  \KwData{this text}
%  \KwResult{how to write algorithm with \LaTeX2e }
%  initialization\;
%  \While{not at end of this document}{
%   read current\;
%   \eIf{understand}{
%   go to next section\;
%   current section becomes this one\;
%   }{
%   go back to the beginning of current section\;
%   }
%  }
%  \caption{How to write algorithms}
% \end{algorithm}

% describe every element in the pipeline
% what is the labeling model

% \paragraph{Labeling model} 


% different strategies

% concatneation; MTL (Multi-task learning)

% MTL -- how to leverage explanations in a supervised setting


\subsection{Learning from unlabeled data}

Besides learning from labeled papers, we can also learn from unlabeled papers. Inspired by the approach democratic co-learning~\cite{zhou2004democratic} which employs inductive biases from models with different inductive biases, and co-training~\cite{blum1977combining} which leverages different views of data representation, we can train two models (\textbf{labeling model} and \textbf{LitGen model}) with the following constraints: 1). Two models cannot have similar architecture; 2). Two models must be trained on different representations of the data. 

\paragraph{Text featurizer} In order to train a labeling model, we need to featurize the papers into a fixed-dimensional representation. Here we use frequency-encoded unigram as the feature representation of the text. By processing the labeled paper dataset and removing stop words, we have 16,860 unique words. For each paper abstract, we construct our unigram feature representation of the abstract by building a 16,860 dimension vector.

% \noindent\textbf{Labeling model} We use a random forest model as our labeling model with the one-hot encoded unigram as the feature representation of the text. By processing the labeled paper dataset and removing stop words, we have 16,860 unique words. For each paper abstract, we construct our unigram feature representation of the abstract by building a 16,860 dimension vector. The process is visualized in Figure~\ref{fig:input-pipeline}.

\paragraph{Labeling model} We use a random forest model with multiple binary output as the learning model that takes the features from the \textbf{text featurizer}.

\paragraph{LitGen model} \james{I thought LitGen refers to the best model which uses the unlabeled data and other tricks. Isn't this biLSTM only the baseline?} is a long-short-term memory network model as described. For each paper abstract, we use an embedding lookup process -- for each word in the abstract, we look up a pre-existing word embedding from a large pre-trained word embedding dictionary GloVe~\cite{pennington2014glove}. For words that are specific to our corpus and cannot be found in GloVe, we initialize the embedding according to the Xavier-uniform distribution~\cite{glorot2010understanding}.
%(the range of this distribution is automatically determined by the dimension of our word embedding and number of vocabulary in our dataset).
%between [-0.0173, 0.0173].

\begin{figure}[h]
\centerline{
\includegraphics[scale=0.5]{images/WeakSupFigure5.pdf} % [width=4.5cm]
}
\caption{The different views of inputs for the labeling model and the LitGen model. Labeling model takes inputs from the text featurizer.}
\label{fig:input-pipeline}
\end{figure}


\begin{figure}[h]
\centerline{
\includegraphics[scale=0.4]{images/WeakSupFigure1.pdf} % [width=4.5cm]
}
\caption{General training pipeline that leverages unlabeled data.}
\label{fig:model-pipeline}
\end{figure}

We train the \textbf{labeling model} on the ClinGen labeled papers once and use it to generate labels for unlabeled papers retrieved by LitVar. Then we train the \textbf{LitGen model} on both noisly labeled papers and ClinGen's ground-truth labeled papers. 

% Subsume everything into proxy-label generating category
% don't write multi-view...because you are not alternating...

%\paragraph{Multi-view training}
% RF + LSTMs

%\paragraph{Weakly supervised training}
% snorkel

% straight-forward training for the LitGen model, MTL, multi-task
% so basically
% without unsupervised data
% with unsuperivsed data

\subsection{Learning from unlabeled data guided by explanations}

Explanations may offer insights on what words are important for the prediction of a VCI tab. This means we can use explanations to find a better set of keywords for the \textbf{text featurizer} module.

We build a logistic regression classifier with lasso loss on the ClinGen Human Explanations dataset. This lasso classifier uses the unigram feature representation of explanations. After removing stop words, the ClinGen Human Explanations dataset has 7,550 unique words. After fully training our lasso classifier, we select words that have non-zero regression coefficients. We are able to select 799 words that are deemed as important predictors for 5 VCI tabs.
%The lasso classifier can achieve 89\% accuracy evaluated on the ClinGen dataset.

% TODO: add the explanations keyword set here (with coefficients). Either build LucidChart, or a table...maybe a table is better.

One advantage of this approach is that by reducing the dimension of the feature representation. This allows our \textbf{labeling model} to have better performance, as we will empirically observe. 

\begin{figure}[h]
\centerline{
\includegraphics[scale=0.7]{images/Keywords.pdf} % [width=4.5cm]
}
\caption{We deisplay a set of keywords that are most positively associated with each VCI tabs from human explanations by training a lasso model on unigram features. Coefficients refer to Lasso coefficients.\james{sufficient to show only two decimal digits for the coefficients.}\anie{addressed!}}
\label{tab:keywords}
\end{figure}

\paragraph{Snorkel-Metal} 
Another advantage is that these keywords can be also used as simple heuristic labeling functions for other weak supervision algorithms such as Snorkel-MeTal~\cite{ratner2018snorkel}.
We show a list of keywords that are most positively associated with each tab in Figure~\ref{tab:keywords}. Keywords selected by lasso have these advantages that fit naturally into Snorkel style labeling functions: 1) We get positive and negaitve keywords as Snorkel labeling functions require both; 2) If no word is found, our labeling function will output N/A (missing), which is required by Snorkel labeling function as well.
